Peak-Age Violation Guarantees for the Transmission of Short Packets over Fading Channels

We investigate the probability that the peak age of information in a point-to-point communication system operating over a multiantenna wireless fading channel exceeds a predetermined value. The packets are scheduled according to a last-come first-serve policy with preemption in service, and are transmitted over the channel using a simple automatic repetition request protocol. We consider quadrature phase shift keying modulation, pilot-assisted transmission, maximum-likelihood channel estimation, and mismatched scaled nearest-neighbor decoding. Our analysis, which exploits nonasymptotic tools in information theory, allows one to determine, for a given information packet size, the physical layer parameters such as the SNR, the number of transmit and receive antennas, the amount of frequency diversity to exploit, and the number of pilot symbols, to ensure that the system operates below a target peak-age violation probability.

==> Inputs/defs.tex <==
\usepackage{bm}
\usepackage{upgreek}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{mathrsfs}
\usepackage{xspace}

\safemath{\mi}{I}
\safemath{\difent}{\mathrm{h}}		%differential entropy
\safemath{\NonnegReal}{\mathbb{R}^{+}}


\safemath{\indist}{\cdfP} %input distribution
\safemath{\outdist}{\cdfQ} %output distribution
\safemath{\inpdf}{\pdfp} %input pdf
\safemath{\outpdf}{\pdfq} %output pdf
\safemath{\testdist}{\cdfP} %the distribution of test P_{Z|W}

%\safemath{\tr}[#1]{\mathrm{tr}\left\lbrace #1  \right\rbrace}

\safemath{\powallocvec}{\vecv}
\safemath{\powalloc}{v}
\safemath{\encoder}{f} % the encoder of the code
\safemath{\decoder}{g} % the decoder of the code
\safemath{\msg}{J} % the message
\safemath{\csir}{\mathrm{r}}
\safemath{\csit}{\mathrm{t}}
\safemath{\csi}{\mathrm{csi}}
\safemath{\csirt}{\mathrm{rt}}
\safemath{\Rcsirt}{R_{\csirt}} %rate with CSIT
\safemath{\Rcsir}{R_{\csir}}
\safemath{\Rcsit}{R_{\csit}}
\safemath{\cohblock}{T}
\safemath{\blocklength}{n}
\safemath{\selbranches}{L}


\safemath{\Rnocsit}{R_{\mathrm{no}}} %rate without CSIT
\safemath{\Rnocsi}{R_{\mathrm{no}}} %rate without CSIT
\safemath{\Rgeneral}{R_{\mathrm{no,rt}}} %rate with general CSI condition
\safemath{\equalR}{R_{\mathrm{e}}}

\newcommand*\pFqskip{8mu}
\catcode`,\active
\newcommand*\pFq{\begingroup
        \catcode`\,\active
        \def ,{\mskip\pFqskip\relax}%
        \dopFq
}
\catcode`\,12
\def\dopFq#1#2#3#4#5{%
        {}_{#1}F_{#2}\biggl[\genfrac..{0pt}{}{#3}{#4};#5\biggr]%
        \endgroup
}

%------------------------------------
%		JOHAN
%------------------------------------
\safemath{\Rmax}{R^*(n,\epsilon)} %rate without CSIT
\safemath{\codewords}{K}
\safemath{\Rub}{\bar{R}(n,\epsilon)}
\safemath{\Rlb}{\underline{R}(n,\epsilon)}
\safemath{\rk}{\kappa}
\safemath{\rlos}{\bar{\matH}}
\safemath{\rnlos}{\tilde{\randmatH}}

\safemath{\randtemp}{K}

\safemath{\Vnocsit}{V_{\error}^{\mathrm{no}}}
\safemath{\Vcsit}{V_{\error}^{\mathrm{rt}}}

\safemath{\cadist}{F_C} %capacity distribution
\safemath{\cdistno}{F_{0}}
\safemath{\cdistcsit}{F_{1}}


\safemath{\deF}{d_0} %the derivative of F_C(\xi) %\left.\frac{d\cadist(\argpn)}{d\argpn}\right|_{\argpn=C_\error}

\safemath{\bl}{n} %block length
\safemath{\blt}{\tilde{\bl}}
\safemath{\error}{\epsilon} %prob of error
\safemath{\NumCode}{M}
\safemath{\RXant}{r}
%\safemath{\rxant}{r}
%\safemath{\txant}{t}
\safemath{\txantop}{t^{\ast}}
\safemath{\minant}{m}
\safemath{\minantop}{\minant^\ast}
\safemath{\snr}{\rho}
\safemath{\const}{k}
\safemath{\inset}{\setF} %the input power set
\safemath{\spanm}{\mathrm{span}}
\safemath{\ubb}{b_{0}}%upper bound of b_1,...,b_{r} of the matrix I+ H^H U H.

%%%%%%%%%%%MIMO%%%%%%%%%%%%%%%%%%%%
\safemath{\covmat}{\matU}
\safemath{\covmatY}{\matV}
\safemath{\randcmY}{\randmatV}

\safemath{\insetMIMO}{\setF_{\txant,\bl}}
\safemath{\insetcov}{\setU_{\txant}}
%\safemath{\condcov}{\matQ\succeq\mathbf{0},\tr(\matQ)\leq\snr}
\safemath{\condcov}{\matQ\in\insetcov}

\safemath{\BoundFU}{k_{\delta}}

\safemath{\argpn}{\xi} % the argument in the probability p(R)

\safemath{\angletest}{Z} %the angle test used in achievability part

\safemath{\Cnocsit}{C_{\epsilon}^{(0)}}
\safemath{\Ccsit}{C_{\epsilon}^{(1)}}

\safemath{\errorach}{P_\mathrm{e}} %the error in intuition part



\newcommand{\given}{\,\vert\,}				% conditioning
\newcommand{\ggiven}{\,\Vert\,}	
\safemath{\define}{\triangleq}			% definition
%\safemath{\fnorm}{\mathrm{F}}

\safemath{\altbl}{\tilde{\bl}}
\safemath{\constL}{k_{\mathrm{L}}}
\safemath{\constU}{k_{\mathrm{U}}}
\safemath{\funcL}{\tilde{q}}
\safemath{\funcU}{q}
\safemath{\ConstThm}{k_0}
%%%%%%%%%%%%%%%%used in the intuition part %%%%%%%%%%%%%
\safemath{\randrevec}{\randvecy}
\safemath{\revec}{\vecy}
\safemath{\trcwd}{\vecx}
\safemath{\randtrcwd}{\randvecx}
\safemath{\randnoisevec}{\randvecw}
\safemath{\transmitcwd}{\vecx_1} %the transmitted codeword in achievability
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%used in the appendix of proving gamma=C_error + O(1/\bl) %%%%%%%%%%%%%
\safemath{\pickcwdnoch}{\vecx_0} %the chosen codeword x=[P,P,...,P]
\safemath{\pickcwd}{\vecx_0} %the chosen codeword x=[P,P,...,P]

\safemath{\inseqrand}{\randvecx}
\safemath{\inseq}{\vecx}

\safemath{\outseq}{\matY}
\safemath{\outseqrand}{\randmatY}

%used in the appendix of the proof of achievability
\safemath{\altT}{\widetilde{T}}
\safemath{\altU}{\widetilde{U}}
\safemath{\altmean}{\tilde{\mu}}
\safemath{\altvar}{\tilde{\sigma}}
\safemath{\altf}{\funcL}
\safemath{\altg}{\tilde{g}}
\safemath{\altgamma}{\tilde{\gamma}}
\safemath{\altdelta}{\tilde{\delta}}
\safemath{\altk}{\tilde{k}}
\safemath{\altconst}{\altk}
\safemath{\altbmLambda}{\widetilde{\bm{\Lambda}}}
\safemath{\constant}{\tilde{k}}


==> Inputs/fig_lambda_var.tex <==
 \begin{tikzpicture}
%/*
\pgfplotsset{
    scaled y ticks = false,
    width=\fwidth*0.45,
    height=\fwidth*0.4,
     title style={yshift=-6pt,}
}
    \begin{groupplot}[
        group style={
        group name = my plots,
        group size=2 by 1,
        vertical sep=45pt,
        horizontal sep=35pt
        },
    ]
    % -------------------------------------------------------------------------------------------------------------------
    % -------------------------------------------------------------------------------------------------------------------
    % -------------------------------------------------------------------------------------------------------------------
    % -------------------------------------------------------------------------------------------------------------------
    % Plot [1, 1]
    % -------------------------------------------------------------------------------------------------------------------
    % -------------------------------------------------------------------------------------------------------------------
    % -------------------------------------------------------------------------------------------------------------------
    % -------------------------------------------------------------------------------------------------------------------
    \nextgroupplot[
        axis x line*=bottom,
        ymode = log,
        xlabel={SNR},
        ylabel = $\epsilon$,
        xmin = -5,
        xmax = 2,
        ymin = 1e-9,
        ymax = 1,
        % xticklabels={{$2$}, {$4$}, {$7$}, {$14$}, {$21$},{$28$}, {$42$},{$84$}},
        % xtick={2, 4 , 7,14,21,28,42, 84},
        % ytick={2, 4 , 6,8,10,12,14},
        xlabel near ticks,
        grid=both,
        legend style={at={($(0,0)+(1cm,1cm)$)},legend columns=3,fill=none,draw=black,anchor=center,align=center},
        legend to name=fred
    ]
 %---------------------------------------------------------------------------------------------------------------------------------------------------
 %                                          DT + MC
 %---------------------------------------------------------------------------------------------------------------------------------------------------
 \addplot [ color=blue!80!black, mark=*,solid, mark size=\marksize,line width=\linew] table [y index={1}, x index = {0}, col sep=comma] {./MATLAB/Noisy Feedback/BIAWGN/Data/Thm1_BIAWGN_EPSILON_VERSUS_SNR_k_30_n_50_Nmax_10_ell_3_eps_1e-3.csv};\addlegendentry{$\nc+\nf=50$}

 \addplot [ color=green!80!black, mark=*,solid, mark size=\marksize,line width=\linew] table [y index={1}, x index = {0}, col sep=comma] {./MATLAB/Noisy Feedback/BIAWGN/Data/Thm1_BIAWGN_EPSILON_VERSUS_SNR_k_30_n_40_Nmax_10_ell_3_eps_1e-3.csv};\addlegendentry{$\nc+\nf=40$}

 \addplot [ color=red!80!black, mark=*,solid, mark size=\marksize,line width=\linew] table [y index={1}, x index = {0}, col sep=comma] {./MATLAB/Noisy Feedback/BIAWGN/Data/Thm1_BIAWGN_EPSILON_VERSUS_SNR_k_30_n_30_Nmax_10_ell_3_eps_1e-3.csv};\addlegendentry{$\nc+\nf=30$}

 \node[] at (axis cs: -3,1e-4) {$\ell = 3$}; %absolute coordinates
 \node[] at (axis cs: -3.35,3e-5) {$\log_2{M} = 30$}; %absolute coordinates
 \node[] at (axis cs: -3.2,1e-5) {$ \nmax= 10$}; %absolute coordinates

    % (Relative) Coordinate at top of the first plot
    \coordinate (c1) at (rel axis cs:0,1);

    % -------------------------------------------------------------------------------------------------------------------
    % -------------------------------------------------------------------------------------------------------------------
    % -------------------------------------------------------------------------------------------------------------------
    % -------------------------------------------------------------------------------------------------------------------
    % Plot [1, 2]
    % -------------------------------------------------------------------------------------------------------------------
    % -------------------------------------------------------------------------------------------------------------------
    % -------------------------------------------------------------------------------------------------------------------
    % -------------------------------------------------------------------------------------------------------------------
    \nextgroupplot[
    	  axis x line*=bottom,
        xlabel={SNR},
        ylabel = $\nf^*$,
        xmin = -5,
        xmax = 2,
        ymin = 1,
        ymax = 15,
        yticklabels={{$1$}, {$5$}, {$10$}, {$15$}},
        % xtick={2, 4 , 7,14,21,28,42, 84},
        ytick={1,5,10,15},
		    legend pos=north west,
        xlabel near ticks,
        grid=both,
    ]
       \addplot [const plot, color=blue!80!black, mark=*,solid, mark size=\marksize,line width=\linew, forget plot] table [y index={2}, x index = {0}, col sep=comma] {./MATLAB/Noisy Feedback/BIAWGN/Data/Thm1_BIAWGN_EPSILON_VERSUS_SNR_k_30_n_50_Nmax_10_ell_3_eps_1e-3.csv};

       \addplot [const plot, color=green!80!black, mark=*,solid, mark size=\marksize,line width=\linew, forget plot] table [y index={2}, x index = {0}, col sep=comma] {./MATLAB/Noisy Feedback/BIAWGN/Data/Thm1_BIAWGN_EPSILON_VERSUS_SNR_k_30_n_40_Nmax_10_ell_3_eps_1e-3.csv};

       \addplot [const plot, color=red!80!black, mark=*,solid, mark size=\marksize,line width=\linew, forget plot] table [y index={2}, x index = {0}, col sep=comma] {./MATLAB/Noisy Feedback/BIAWGN/Data/Thm1_BIAWGN_EPSILON_VERSUS_SNR_k_30_n_30_Nmax_10_ell_3_eps_1e-3.csv};


        % (Relative) Coordinate at top of the second plot
    \coordinate (c2) at (rel axis cs:1,1);% I moved this to the upper right corner

\end{groupplot}

\coordinate (c3) at ($(c1)!.5!(c2)$);
\node[above] at (c3 |- current bounding box.north)
{\pgfplotslegendfromname{fred}};

\node[text width=6cm,align=center,anchor=north,font=\footnotesize] at ([yshift=-5mm]my plots c1r1.south) {\subcaption{Minimum error probability optimized over $\nc$ and $\nf$.\label{fig:BIAWGN_b1}}};
\node[text width=6cm,align=center,anchor=north,font=\footnotesize] at ([yshift=-5mm]my plots c2r1.south) {\subcaption{Optimal number of resources over the feedback channel. \label{fig:BIAWGN_b2}}};
\end{tikzpicture}%

